Long or short CoT? Investigating Instance-level Switch of Large Reasoning Models

With the rapid advancement of large reasoning models, long Chain-of-Thought (CoT) prompting has demonstrated strong performance on complex tasks. However, this often comes with a significant increase in token usage. In this paper, we conduct a comprehensive empirical analysis comparing long and short CoT strategies. Our findings reveal that while long CoT can lead to performance improvements, its benefits are often marginal relative to its significantly higher token consumption. Specifically, long CoT tends to outperform when ample generation budgets are available, whereas short CoT is more effective under tighter budget constraints. These insights underscore the need for a dynamic approach that selects the proper CoT strategy based on task context and resource availability. To address this, we propose SwitchCoT, an automatic framework that adaptively chooses between long and short CoT strategies to balance reasoning accuracy and computational efficiency. Moreover, SwitchCoT is designed to be budget-aware, making it broadly applicable across scenarios with varying resource constraints. Experimental results demonstrate that SwitchCoT can reduce inference costs by up to 50% while maintaining high accuracy. Notably, under limited token budgets, it achieves performance comparable to, or even exceeding, that of using either long or short CoT alone.

==> fig/fig.tex <==
% \begin{figure}
%   \centering
%   \includegraphics[width=0.8\textwidth]{srcs/improve.pdf}
%   \caption{improvement}
%   \label{fig:improve}
% \end{figure}

% \begin{figure}
%   \centering
%   \includegraphics[width=0.5\textwidth]{srcs/improve.pdf}
%   \caption{dot}
%   \label{fig:dot}
% \end{figure}

% \begin{figure}
%   \centering
%   \includegraphics[width=1\textwidth]{srcs/improve.pdf}
%   \caption{dotall}
%   \label{fig:dotall}
% \end{figure}



\begin{figure}[]
  \centering
    \subfigure[1]{
        \centering
        \includegraphics[width=0.9\textwidth]{srcs/improve.pdf}
        \label{fig:improve}
    }
     \subfigure[2]{
        \includegraphics[width=0.45\textwidth]{srcs/dot.pdf}
        \label{fig:dot}
    }
     \subfigure[3]{
        \includegraphics[width=0.45\textwidth]{srcs/dotall.pdf}
        \label{fig:dotall}
    }
    
  \caption{level}
  \label{fig:level}
\end{figure}




\begin{figure}
  \centering
    \subfigure[level1]{
        \includegraphics[width=0.45\textwidth]{srcs/level1.pdf}
    }
     \subfigure[level2]{
        \includegraphics[width=0.45\textwidth]{srcs/level2.pdf}
    }
     \subfigure[level3]{
        \includegraphics[width=0.45\textwidth]{srcs/level3.pdf}
    }
     \subfigure[level4]{
        \includegraphics[width=0.45\textwidth]{srcs/level4.pdf}
    }
    
  \caption{level}
  \label{fig:level}
\end{figure}



\begin{figure}[htbp]
  \centering

  % 左边图：3×1
  \begin{minipage}[t]{0.22\textwidth}
    \centering
    \subfigure[MATH]{
        \includegraphics[width=0.7\linewidth]{srcs/matrix/matrix1.pdf}
    }\\
    \subfigure[Knowledge]{
        \includegraphics[width=0.7\linewidth]{srcs/matrix/matrix2.pdf}
    }\\
    \subfigure[Social]{
        \includegraphics[width=0.7\linewidth]{srcs/matrix/matrix3.pdf}
    }
    \caption{left}
    \label{fig:matrix level}
  \end{minipage}
  \hfill
  % 右边图：2×4
  \begin{minipage}[t]{0.7\textwidth}
  \vspace*{3em}
    \centering
    \subfigure[\scriptsize{GSM8K}]{
        \includegraphics[width=0.22\linewidth]{srcs/matrix/matrix21.pdf}
    }
    \subfigure[\scriptsize{MATH500}]{
        \includegraphics[width=0.22\linewidth]{srcs/matrix/matrix22.pdf}
    }
    \subfigure[\scriptsize{AMC23}]{
        \includegraphics[width=0.22\linewidth]{srcs/matrix/matrix23.pdf}
    }
    \subfigure[\scriptsize{AIME25}]{
        \includegraphics[width=0.22\linewidth]{srcs/matrix/matrix24.pdf}
    }\\[1ex]
    \subfigure[\scriptsize{ARC-easy}]{
        \includegraphics[width=0.22\linewidth]{srcs/matrix/matrix31.pdf}
    }
    \subfigure[\scriptsize{ARC-challenge}]{
        \includegraphics[width=0.22\linewidth]{srcs/matrix/matrix32.pdf}
    }
    \subfigure[\scriptsize{MMLU}]{
        \includegraphics[width=0.22\linewidth]{srcs/matrix/matrix33.pdf}
    }
    \subfigure[\scriptsize{GPQA}]{
        \includegraphics[width=0.22\linewidth]{srcs/matrix/matrix34.pdf}
    }
    \caption{Right}
    \label{fig:matrix sizes}
  \end{minipage}

\end{figure}



\begin{figure}
  \centering
  \subfigure[\scriptsize{GSM8K}]{
        \includegraphics[width=0.23\textwidth]{srcs/budget/budget1.pdf}
    }
    \subfigure[\scriptsize{MATH500}]{
        \includegraphics[width=0.23\textwidth]{srcs/budget/budget2.pdf}
    }
    \subfigure[\scriptsize{AMC23}]{
        \includegraphics[width=0.23\textwidth]{srcs/budget/budget3.pdf}
    }
    \subfigure[\scriptsize{AIME25}]{
        \includegraphics[width=0.23\textwidth]{srcs/budget/budget4.pdf}
    }
    \subfigure[\scriptsize{ARC-easy}]{
        \includegraphics[width=0.23\textwidth]{srcs/budget/budget5.pdf}
    }
    \subfigure[\scriptsize{ARC-challenge}]{
        \includegraphics[width=0.23\textwidth]{srcs/budget/budget6.pdf}
    }
    \subfigure[\scriptsize{MMLU}]{
        \includegraphics[width=0.23\textwidth]{srcs/budget/budget7.pdf}
    }
    \subfigure[\scriptsize{GPQA}]{
        \includegraphics[width=0.23\textwidth]{srcs/budget/budget8.pdf}
    }
  \caption{budget}
  \label{fig:budget}
\end{figure}



\begin{figure}
  \centering
  \subfigure[\scriptsize{1}]{
        \includegraphics[width=0.7\textwidth]{srcs/experience/exp1.pdf}
    }
    \subfigure[\scriptsize{2}]{
        \includegraphics[width=0.31\textwidth]{srcs/experience/exp2.pdf}
    }
    \subfigure[\scriptsize{3}]{
        \includegraphics[width=0.31\textwidth]{srcs/experience/exp3.pdf}
    }

    \caption{experience}
    \label{fig:experience}

\end{figure}


\begin{figure}
  \centering
  \includegraphics[width=0.7\textwidth]{srcs/method.pdf}
  \caption{method}
  \label{fig:method}
\end{figure}

==> fig/figall.tex <==
\begin{figure}[]
  \centering
    \subfigure[The improvement of long CoT over short CoT]{
         \includegraphics[width=0.6\textwidth]{srcs/improve.pdf}
    }
     \subfigure[11]{
         \includegraphics[width=0.3\textwidth]{srcs/dotall.pdf}
    }

       
  \label{fig:all}
\end{figure}

% The improvement of long CoT 对比short CoT. 

==> fig/figbudget.tex <==
\begin{figure}
  \centering
  \subfigure[\scriptsize{GSM8K}]{
        \includegraphics[width=0.23\textwidth]{srcs/budget/budget1.pdf}
    }
    \subfigure[\scriptsize{MATH500}]{
        \includegraphics[width=0.23\textwidth]{srcs/budget/budget2.pdf}
    }
    \subfigure[\scriptsize{AMC23}]{
        \includegraphics[width=0.23\textwidth]{srcs/budget/budget3.pdf}
    }
    \subfigure[\scriptsize{AIME25}]{
        \includegraphics[width=0.23\textwidth]{srcs/budget/budget4.pdf}
    }
    \subfigure[\scriptsize{ARC-easy}]{
        \includegraphics[width=0.23\textwidth]{srcs/budget/budget5.pdf}
    }
    \subfigure[\scriptsize{ARC-challenge}]{
        \includegraphics[width=0.23\textwidth]{srcs/budget/budget6.pdf}
    }
    \subfigure[\scriptsize{MMLU}]{
        \includegraphics[width=0.23\textwidth]{srcs/budget/budget7.pdf}
    }
    \subfigure[\scriptsize{GPQA}]{
        \includegraphics[width=0.23\textwidth]{srcs/budget/budget8.pdf}
    }
  \caption{\textbf{Accuracy between long and short CoT under different token budgets.}They are conducted on the Deepseek-distill-Qwen-7B model. }
  \label{fig:budget}
\end{figure}


% on the Deepseek-distill-Qwen-7B model
% 不同token预算下长短cot准确率的比较，

==> fig/figexp.tex <==
\begin{figure}
  \centering
  \subfigure[\scriptsize{All Samples}]{
        \includegraphics[width=0.3\textwidth]{srcs/experience/exp1.pdf}
    }
    \subfigure[\scriptsize{MATH}]{
        \includegraphics[width=0.3\textwidth]{srcs/experience/exp2.pdf}
    }
    \subfigure[\scriptsize{Knowledge}]{
        \includegraphics[width=0.3\textwidth]{srcs/experience/exp3.pdf}
    }

    \caption{\textbf{Experiment results under different token budge.} The red line represents our method. It consistently achieves the best performance across different token budgets. }
    \label{fig:experience}

\end{figure}

==> fig/figlevel.tex <==
\begin{figure}
  \centering
    \subfigure[Math]{
        \includegraphics[width=0.4\textwidth]{srcs/level1.pdf}
    }
     \subfigure[Knowledge]{
        \includegraphics[width=0.4\textwidth]{srcs/level2.pdf}
    }
    
  \caption{level}
  \label{fig:level}
\end{figure}


% the improvement on different difficult level on math problems

==> fig/figmatrix.tex <==
% \begin{figure}[t]
%   \centering

%   % 左边图：3×1
%   \begin{minipage}[t]{0.18\textwidth}
%     \centering
%     \subfigure[MATH]{
%         \includegraphics[width=0.7\linewidth]{srcs/matrix/matrix1.pdf}
%     }\\
%     \subfigure[Knowledge]{
%         \includegraphics[width=0.7\linewidth]{srcs/matrix/matrix2.pdf}
%     }\\
%     \subfigure[Social]{
%         \includegraphics[width=0.7\linewidth]{srcs/matrix/matrix3.pdf}
%     }
%     \caption{left}
%     \label{fig:matrix level}
%   \end{minipage}
%   \hfill
%   % 右边图：2×4
%   \begin{minipage}[t]{0.7\textwidth}
%   \vspace*{3em}
%     \centering
%     \subfigure[\scriptsize{GSM8K}]{
%         \includegraphics[width=0.18\linewidth]{srcs/matrix/matrix21.pdf}
%     }
%     \subfigure[\scriptsize{MATH500}]{
%         \includegraphics[width=0.18\linewidth]{srcs/matrix/matrix22.pdf}
%     }
%     \subfigure[\scriptsize{AMC23}]{
%         \includegraphics[width=0.18\linewidth]{srcs/matrix/matrix23.pdf}
%     }
%     \subfigure[\scriptsize{AIME25}]{
%         \includegraphics[width=0.18\linewidth]{srcs/matrix/matrix24.pdf}
%     }\\[1ex]
%     \subfigure[\scriptsize{ARC-easy}]{
%         \includegraphics[width=0.18\linewidth]{srcs/matrix/matrix31.pdf}
%     }
%     \subfigure[\scriptsize{ARC-challenge}]{
%         \includegraphics[width=0.18\linewidth]{srcs/matrix/matrix32.pdf}
%     }
%     \subfigure[\scriptsize{MMLU}]{
%         \includegraphics[width=0.18\linewidth]{srcs/matrix/matrix33.pdf}
%     }
%     \subfigure[\scriptsize{GPQA}]{
%         \includegraphics[width=0.18\linewidth]{srcs/matrix/matrix34.pdf}
%     }
%     \caption{Right}
%     \label{fig:matrix sizes}
%   \end{minipage}

% \end{figure}



\begin{figure}
    \centering
    
  \subfigure[MATH]{
        \includegraphics[width=0.2\linewidth]{srcs/matrix/matrix1.pdf}
    }
    \hspace{1em}
    \subfigure[Knowledge]{
        \includegraphics[width=0.2\linewidth]{srcs/matrix/matrix2.pdf}
    }
    \hspace{1em}
    \subfigure[Social]{
        \includegraphics[width=0.2\linewidth]{srcs/matrix/matrix3.pdf}
    }
    
    \caption{\textbf{Confusion matrices across different data types.} Each matrix is averaged over all datasets belonging to the same data type and further averaged across different models.}
    \label{fig:matrix level}
\end{figure}

% 在不同数据类型下的混淆矩阵，每一个数据类型是由数据集是取平均值得到的，也是由不同的模型取平均得到的




==> fig/figmatrixhow.tex <==

\begin{wrapfigure}{r}{0.3\textwidth}
    \centering
    \includegraphics[width=0.8\linewidth]{srcs/matrix/matrix.pdf}
    \caption{Caption}
    \label{fig:matrix}
\end{wrapfigure}

==> fig/figmethod.tex <==




% \begin{figure}[t]
%   \centering
%   \begin{minipage}[t]{0.48\textwidth}
%     \vspace{0pt}  % 强制顶对齐
%     \centering
%     \includegraphics[width=\linewidth]{srcs/prompt.pdf}
%     \caption{Prompt}
%     \label{fig:prompt}
%   \end{minipage}
%   \hfill
%   \begin{minipage}[t]{0.48\textwidth}
%     \vspace{15pt}  % 强制顶对齐
%     \centering
%     \includegraphics[width=\linewidth]{srcs/method.pdf}
%     \caption{method }
%     \label{fig:method}
%   \end{minipage}
% \end{figure}

% 我们方法的工作流程，给定一个问题，AutoSCoT先经过stageI寻找最优的回答策略。在stageII，AutoSCoT使用选择好的回答策略生成答案。


\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{srcs/method.pdf}
    \caption{\textbf{The workflow of AutoSCoT.} Given a question, it first selects the optimal reasoning strategy using a fine-tuned selector model (Stage\uppercase\expandafter{\romannumeral1}). Then in Stage\uppercase\expandafter{\romannumeral2},  it employs a base language model to generate the answer based on the selected strategy.}
    \label{fig:method}
\end{figure}


==> fig/figsize.tex <==
\begin{figure}[]
  \centering
     \subfigure[Math]{
        \includegraphics[width=0.3\textwidth]{srcs/dot/dotmath.pdf}
    }
     \subfigure[Knowledge]{
        \includegraphics[width=0.3\textwidth]{srcs/dot/dotknow.pdf}
    }
    \subfigure[Social]{
        \includegraphics[width=0.3\textwidth]{srcs/dot/dotsoc.pdf}
    }
  \caption{level}
  \label{fig:level}
\end{figure}

==> fig/tablemarix.tex <==


\begin{table}[t]
    \centering
    \begin{minipage}[t]{0.4\textwidth}
        \centering
        \begin{tabular}{c|c|c}
            \toprule
          & False-True & True-False  \\
        \midrule
        GSM8K & 9.9 & 2.2  \\
        MATH500 & 14.5 & 2.0  \\
        AMC23 & 18.6 & 2.5  \\
        AIME25 & 20.2 & 4.9  \\
            \bottomrule
        \end{tabular}
        \vspace{1em}
        \caption{Left Table}
        \label{tab:left}
    \end{minipage}
    \label{tab:matrix math}
    \hfill
    % \hspace{3em} % 控制间距
    \begin{minipage}[t]{0.4\textwidth}
        \centering
        \begin{tabular}{c|c|c}
            \toprule
            & False-True & True-False  \\
            \midrule
            ARC-easy & 4.7 & 1.6 \\
            ARC-challenge & 7.6 & 2.9 \\
            MMLU & 10.7 & 5.7 \\
            GPQA & 17.3 & 10.1 \\
            \bottomrule
        \end{tabular}
        \vspace{1em}
        \caption{Right Table}
        \label{tab:matrix know}
    \end{minipage}
\end{table}




==> srctex/level.tex <==

\begin{figure}
    \centering
    \subfigure[Math]{
        \includegraphics[width=0.43\linewidth]{srcs/fig/level1.pdf}
    }
    \subfigure[Knowledge]{
        \includegraphics[width=0.43\linewidth]{srcs/fig/level2.pdf}
    }
    \caption{Performance gain and token consumption from different difficulty levels}
    \label{fig:level}
\end{figure}

==> srctex/modelscale.tex <==


\begin{wrapfigure}{r}{0.45\textwidth}
    \centering
    \includegraphics[width=1\linewidth]{srcs/fig/modelscale.pdf}
    \caption{The trade-off between token consumption and accuracy for short and long CoT across different datasets and models. Each arrow represents the transition from short CoT to long CoT.}
    \label{fig:modelscale}
\end{wrapfigure}

% 长cot在不同模型不同数据集上的提升，我们的模型都是ds蒸馏系列

% 长短cot在不同数据集不同模型上的token与准确率的，箭头代表从短cot到长cot
